Analytical parametrization and shape classification of anomalous HH production in the EFT approach

In this document we study the effect of anomalous Higgs boson couplings on non-resonant pair production of Higgs bosons ($HH$) at the LHC. We explore the space of the five parameters $\kappa_{\lambda}$, $\kappa_{t}$, $c_2$, $c_g$, and $c_{2g}$ in terms of the corresponding kinematics of the final state, and describe a partition of the space into a limited number of regions featuring similar phenomenology in the kinematics of $HH$ final state. We call clusters the sets of points belonging to the same region; to each cluster corresponds a representative point which we call a benchmark. We discuss a possible technique to estimate the sensitivity of an experimental search to the kinematical differences between the phenomenology of the benchmark points and the rest of the parameter space contained in the corresponding cluster. We also provide an analytical parametrization of the cross-section modifications that the variation of anomalous couplings produces with respect to standard model $HH$ production along with a recipe to translate the results into other parameter-space bases. Finally, we provide a preliminary analysis of variations in the topology of the final state within each region based on recent LHC results.

==> shape.tex <==
\section{Kinematic clustering}
\label{sec:shape}

\subsection{Clustering procedure}
\label{sec:clus}

An important consequence of the introduction of the five BSM parameters in the Lagrangian provided in Eq.~(\ref{eq:lag}), in addition to the modification of the overall Higgs boson pair-production cross section, is the generation of significant modifications of the kinematic properties of the final state with respect to the pure SM process. The experimental exploration of the five-dimensional model space is by no means trivial, as the optimization of the search strategy for the $\HH$ signal depends significantly on the investigated parameter space point. 
In order to address this problem, we designed a clustering procedure to group regions of parameter space which can be probed by the same search. In the spirit of this approach, analyses would optimize their selection for a model (a benchmark) chosen to represent at best the kinematic characteristics of the corresponding region. The benchmarks resulting from the clustering procedure are summarized in this note; for implementation details the reader is referred to  Ref.~\cite{Dall'Osso:2015aia}. We recall below the basic ideas of our procedure.

The  $gg \rightarrow \HH$ production is a $2 \rightarrow 2$ process. 
In the center-of-mass reference frame the kinematic properties of the final state can be fully characterized by two variables: the invariant mass of the two Higgs bosons $\mHH$ and the polar angle of one of the bosons in the center-of-momentum frame $|\cos \theta^{*}|$. At leading order, all other observables describing the final state have no connection to the structure of the Lagrangian density from Eq.~\ref{eq:lag}.
% The probability density function
%of the kinematical quantities do not depend on the EFT parameters.
%In particular,  rapidity of the di-Higgs system
%only depends on the parton distribution functions, which are the same for all
%$gg \rightarrow hh$ processes; and
The kinematic properties of each EFT point can then be characterized by
estimating the two-dimensional probability density function of $\mHH$ and
$|\cos \theta^{*}|$. By using a suitable test statistic sensitive to
the shape differences of the two-dimensional density function, one may quantify
the kinematic differences between different model points in the
five-dimensional phase-space. The value of the test statistic may then be used
to group the models that are kinematically most similar.
This procedure is referred to as \textit{cluster analysis} and a group of models as \textit{a cluster}. The employed test statistic was a likelihood ratio based on Poisson counts in $\mHH-|\cos \theta^{*}|$ histograms; the clustering was performed through a hierarchical agglomerative technique.

The clustering procedure was applied to a set of models corresponding to a fine
scan in several parameter space directions. The investigated range of the parameters was decided by taking into account the current experimental constraints. In particular, the parameters were allowed to
vary as $|\kappa_{\lambda}| \leq$ 15,  $\kappa_t\subset [0.5,2.5]$,  $|c_2| \leq$3 and $(|c_g|,|c_{2g}|) \leq 1$, where $\kappa_t$ and $c_2$ feature a step size of O(0.5) and $\kappa_{\lambda}$ is varied in O(1) steps.
The granularity of the scan in $c_g$ and $c_{2g}$ is 0.2. To have a better accuracy
in the points of minimal di-Higgs production
cross section, where the changes in kinematics are particularly strong, we increased the density of scanned points in the corresponding regions. 
This resulted in a total of 1507 inspected points, distributed with a variable binning within the boundaries quoted above. The
simulations were performed with the Madgraph\_aMC@NLO version 2.2.1 Monte Carlo (MC) simulation package~\cite{Alwall:2014hca}, using the model provided
by the authors of~\cite{Hespel:2014sla}, were the loop factors including the full $m_{t}$
dependence are calculated on an event-by-event basis with a Fortran routine. The PDF set
used was NNPDF23LO1~\cite{Ball:2012cx} and the factorization and renormalization scale considered were
$\sqrt{\hat{s}}= \mHH$. The relevant input masses were $\mH$ = 126\,GeV
and $m_t$ = 173.18\,GeV.

The cluster analysis leads to the division of the 1507 inspected points into 12 groups. Each group displays similar kinematic characteristics, and clear differences compared with members of the other groups. For each cluster a benchmark is defined as the sample most similar to all the others in the cluster, where the similarity metric is the one given by the test statistic. The numerical details are provided later in sub-section~\ref{clus_res}.

\subsection{Outliers}
\label{sec:intra_outliers}

The benchmarks are chosen to capture well the main features of the cluster kinematics. Nevertheless some of the cluster members
still exhibit residual differences with respect to the benchmark. 
These intra-cluster differences could lead to limited deviations
in the experimental signal efficiencies. If the analysis has a sufficient resolution to resolve those differences we propose here a simple approach to select six extreme cases (referred to as outliers) within each
cluster, which can tentatively be used to evaluate the possible variation of experimental efficiencies within a cluster. If the analyzers want to preserve the simplifications offered by the cluster approach we recommend to fully simulate (generate and propagate through the experimental apparatus) only the benchmark and obtain the outliers through an event-by-event reweighing procedure in the $\mHH-|\cos \theta^{*}|$ space. The results (for example limits) shall be then presented for the benchmark and benchmark reweighted to the outliers. The weights may be easily estimated at generator level.

The $\mHH$ distribution features the largest intra-cluster
variation and it is likely the most important distribution
for experimental analyses. We define therefore the outliers as subset of samples that envelope
all the other samples of the cluster in three mass points\footnote{Note that the chosen outliers are susceptible to a different level of
arbitrariness: the choice of the points of the parameter space scan,
the choice of the variable and the points where to search for the cluster
envelope and the histogram binning.} $m_{\rm HH\,,1}\,\equiv$ 270\,GeV,
$m_{\rm HH\,,2}\,\equiv$ 400\,GeV and $m_{\rm HH\,,3}\,\equiv$ 600\,GeV, applied to a histogram with 20\,GeV
wide bins. The first and last mass points are intended to catch
the analysis sensitivity to threshold region ($\mHH \approx 2 m_{\PH}$) and energy-tail modifications. The
intermediate mass point is close to the typical valley found
in the distribution due to a cancellation between the different diagrams, and it is intended
to catch the analyses sensitivity to short-distance fluctuations in shape.
%In Figure~\ref{fig:app_out_mhh} the example of the Cluster 1 is shown. In  Figure~\ref{fig:out_mass} (bottom) you can 
Figure \ref{fig:out_mass} (top) shows an example of the di-Higgs mass distribution for cluster 3 with the outliers.
In Fig.~\ref{fig:out_mass} (bottom) we provide the $\pTH$ and $|\cos \theta^{*}|$ spectra with the same outliers.
One may observe that the choice of outliers in $\mHH$ is also reasonably valid for the two other distributions.

\begin{figure*}[h]\begin{center}
\includegraphics[width=0.41\textwidth, angle =0 ]{envelope/5par_13Tev_Nclu12_Clus3_mhh.pdf}
\includegraphics[width=0.41\textwidth, angle =0 ]{envelope/5par_13Tev_Nclu12_Clus3_pt.pdf}
\includegraphics[width=0.41\textwidth, angle =0 ]{envelope/5par_13Tev_Nclu12_Clus3_hcths.pdf}
\caption{\small  The $\mHH$ (top left), $\pTH$ (top right) and $|\cos \theta^{*}|$ (bottom) distributions for the members of cluster 3. The benchmark (in black color) and corresponding outliers (colored lines) are highlighted. The three mass regions are indicated by vertical dashed lines.\label{fig:out_mass}}
\end{center}\end{figure*}

\subsection{Results}
\label{clus_res}

The list of benchmarks is given in Table \ref{tab:bench}. We recommend the 12 benchmarks listed there to be the parameter space points targeted by experimental searches, in addition to the SM point. Fig.~\ref{fig:app_out_mhh} shows the $\mHH$ spectra for all the clusters together with the outliers, while Table~\ref{tab:out} provides the parameters of all the 72 outliers.

\begin{table}[h]
\centering
\small{
\begin{tabular}{r r r r r r r}
\toprule
Benchmark & $\kappa_{\lambda}$ & $\kappa_{t}$ & $c_{2}$	& $c_{g}$ & $c_{2g}$ \\
\midrule
1 &	7.5	 & 1.0	 &	-1.0	& 0.0	& 0.0 \\
2 &	1.0	 & 1.0	 &	0.5	& -0.8	& 0.6 \\
3 &	1.0	 & 1.0	 &	-1.5	& 0.0	& -0.8 \\
4 &	-3.5     & 1.5   &	-3.0	& 0.0	& 0.0 \\
5 &	1.0	 & 1.0	 &	0.0	& 0.8	& -1.0 \\
6 &	2.4	 & 1.0	 &	0.0	& 0.2	& -0.2 \\
7 &	5.0	 & 1.0	 &	0.0	& 0.2	& -0.2 \\
8 &	15.0     & 1.0	 &	0.0	& -1.0	& 1.0 \\
9 &	1.0	 & 1.0	 &	1.0	& -0.6	& 0.6 \\
10 &	10.0     & 1.5   &	-1.0	& 0.0	& 0.0 \\
11 &	2.4	 & 1.0	 &	0.0	& 1.0	& -1.0 \\
12 &	15.0     & 1.0	 &	1.0	& 0.0	& 0.0 \\ \midrule %cl no. 463
SM &	1.0      & 1.0	 &	0.0	& 0.0	& 0.0 \\
\bottomrule
\end{tabular}
}
\caption{\small Parameter values of the final benchmarks selected by the clustering procedure \cite{Dall'Osso:2015aia}. The third cluster is the one that contains the SM sample (defined by $\kappa_{\lambda}$ = $\kappa_{t}$ =1, $c_{2}$ = $c_{g}$ = $c_{2g}$ = 0). \label{tab:bench}}
\end{table}

Three of the clusters have benchmarks that do not obey the linear EFT  relation, however this does not present a problem for the interpretation of the results, assuming the latter. The phenomenological properties of parameter points within these clusters that belong to the linear realization of EWSB are still well approximated by the corresponding benchmarks.

Relevant properties of those three clusters are described below:
\begin{itemize}
\item In the scan we performed, Cluster 2 does not have representatives in the linear theory. The $\mHH$ extends above the TeV scale - therefore particular caution should be taken when interpreting the experimental results derived for the corresponding benchmark in the EFT (see Fig.~\ref{fig:app_out_mhh}). 

\item Cluster 3 includes the SM point and a large fraction of the points where only $\kappa_{\lambda}$ and $\kappa_t$ are modified, while the coefficients related to purely BSM operators are constrained to 0. 

\item Cluster 5 exhibits a doubly peaked structure in
$\mHH$, corresponding to maximal interference pattern and
associated with regions of minimal cross sections, which also
includes points of the linear case (see Fig.~\ref{fig:app_out_mhh}).

\end{itemize}



\begin{figure}[hbt]\begin{center}
\includegraphics[width=0.32\textwidth, angle =0 ]{envelope/5par_13Tev_Nclu12_Clus1_mhh.png}
\includegraphics[width=0.32\textwidth, angle =0 ]{envelope/5par_13Tev_Nclu12_Clus2_mhh.png}
\includegraphics[width=0.32\textwidth, angle =0 ]{envelope/5par_13Tev_Nclu12_Clus3_mhh.png}
\includegraphics[width=0.32\textwidth, angle =0 ]{envelope/5par_13Tev_Nclu12_Clus4_mhh.png}
%
\includegraphics[width=0.32\textwidth, angle =0 ]{envelope/5par_13Tev_Nclu12_Clus5_mhh.png}
\includegraphics[width=0.32\textwidth, angle =0 ]{envelope/5par_13Tev_Nclu12_Clus6_mhh.png}
\includegraphics[width=0.32\textwidth, angle =0 ]{envelope/5par_13Tev_Nclu12_Clus7_mhh.png}
\includegraphics[width=0.32\textwidth, angle =0 ]{envelope/5par_13Tev_Nclu12_Clus8_mhh.png}
%
\includegraphics[width=0.32\textwidth, angle =0 ]{envelope/5par_13Tev_Nclu12_Clus9_mhh.png}
\includegraphics[width=0.32\textwidth, angle =0 ]{envelope/5par_13Tev_Nclu12_Clus10_mhh.png}
\includegraphics[width=0.32\textwidth, angle =0 ]{envelope/5par_13Tev_Nclu12_Clus11_mhh.png}
\includegraphics[width=0.32\textwidth, angle =0 ]{envelope/5par_13Tev_Nclu12_Clus12_mhh.png}
\caption{\small The $\mHH$ distributions for the 12 clusters. The benchmark (in black color) and corresponding outliers (colored lines) are highlighted. The mass points $\mHH^1$, $\mHH^2$ and $\mHH^3$ are indicated by vertical dashed lines.
 \label{fig:app_out_mhh}}
\end{center}\end{figure}



\begin{table}[h]
\centering
\footnotesize{
\begin{tabular}{|r r r r r|r r r r r|r r r r r|}
\toprule
 \multicolumn{5}{c}{Cluster 1} & \multicolumn{5}{c}{Cluster 2} & \multicolumn{5}{c}{Cluster 3}  \\[1mm] \hline
 $\kappa_{\lambda}$ & $\kappa_{t}$ & $c_2$ & $c_g$ & $c_{2g}$ & $\kappa_{\lambda}$& $\kappa_{t}$ & $c_2$ & $c_g$ & $c_{2g}$& $\kappa_{\lambda}$& $\kappa_{t}$ & $c_2$ & $c_g$ & $c_{2g}$ \\
 15.0  & 1.0 & -3.0 & 0.0 & 0.0   & 1.0 & 1.0 & 0.5 & 1.0 & 0.8   & -10.0 & 0.5 & 3.0 & 0.0 & 0.0 \\
 15.0  & 1.0 & -3.0 & 0.0 & 0$^{*}$ & 1.0 & 1.0 & 0.5 & 0.8 & 0.8 & 5.0 & 1.5 & -2.0 & 0.0 & 0.0 \\
 1.0   & 1.0 & 0.5  & 1.0 & 0.4   & 1.0 & 1.0 & 0.5 & -0.6 & 0.4  & 2.4 & 1.0 & -0.5 & 0.0 & 0.0 \\
 1.0   & 1.0 & 0.5  & 1.0 & 0.2   & 1.0 & 1.0 & 0.5 & -0.8 & 0.4  & 2.4 & 2.0 & 1.0 & 0.0 & 0.0 \\
 15.0  & 1.5 & -3.0 & 0.0 & 0.0   & 1.0 & 1.0 & 0.5 & -1.0 & 0.8  & 2.4 & 2.5 & 1.0 & 0.0 & 0.0 \\
 -10.0 & 0.5 & 1.0  & 0.0 & 0.0   & 1.0 & 1.0 & 0.5 & -1.0 & 1.0  & 1.0 & 2.5 & 1.5 & 0.0 & 0.0 \\\midrule
   \multicolumn{5}{c}{Cluster 4} & \multicolumn{5}{c}{Cluster 5} & \multicolumn{5}{c}{Cluster 6}  \\[1mm] \midrule
 $\kappa_{\lambda}$& $\kappa_{t}$ & $c_2$ & $c_g$ & $c_{2g}$ & $\kappa_{\lambda}$& $\kappa_{t}$ & $c_2$ & $c_g$ & $c_{2g}$& $\kappa_{\lambda}$& $\kappa_{t}$ & $c_2$ & $c_g$ & $c_{2g}$ \\
 5.0 & 2.0 & 3.0 & 0.0 & 0.0 & 5.0 & 1.0 & 0.0 & -0.6 & 0.6 & 10.0 & 2.5 & -2.0 & 0.0 & 0.0 \\
 1.0 & 1.5 & 3.0 & 0.0 & 0.0 & 1.0 & 1.0 & 0.5 & 1.0 & 0.6 & 5.0 & 1.0 & -0.5 & 0.0 & 0.0 \\
 1.0 & 1.0 & 2.0 & 0.0 & -0.4 & 1.0 & 1.0 & 0.0 & 0.2 & -0.8 & 7.5 & 1.5 & -1.0 & 0.0 & 0.0 \\
 1.0 & 1.0 & 0.0 & 0.4 & 0.6 & 1.0 & 1.0 & 0.5 & -1.0 & 0.2 & 2.4 & 1.0 & 0.0 & 0.4 & -0.4 \\
 1.0 & 1.0 & 0.0 & -0.2 & 0.4 & -2.4 & 1.5 & 2.0 & 0.0 & 0.0 & 5.0 & 2.5 & 1.0 & 0.0 & 0.0 \\
 -2.4 & 1.0 & 0.0 & -0.6 & 0.6 & -2.4 & 1.0 & 1.0 & 0.0 & 0.0 & 5.0 & 1.75 & 0.0 & 0.0 & 0.0 \\\midrule
  \multicolumn{5}{c}{Cluster 7} & \multicolumn{5}{c}{Cluster 8} & \multicolumn{5}{c}{Cluster 9}  \\[1mm] \midrule
   $\kappa_{\lambda}$& $\kappa_{t}$ & $c_2$ & $c_g$ & $c_{2g}$ & $\kappa_{\lambda}$& $\kappa_{t}$ & $c_2$ & $c_g$ & $c_{2g}$& $\kappa_{\lambda}$& $\kappa_{t}$ & $c_2$ & $c_g$ & $c_{2g}$ \\
 10.0 & 2.5 & 2.0 & 0.0 & 0.0 & 7.5 & 2.5 & -1.0 & 0.0 & 0.0 & 10.0 & 0.5 & -2.0 & 0.0 & 0.0 \\
 15.0 & 0.5 & 0.0 & 0.0 & 0.0 & 3.5 & 2.0 & 0.5 & 0.0 & 0.0 & 1.0 & 1.0 & 0.0 & -0.2 & -0.4 \\
 15.0 & 0.5 & 0.0 & 0.0 & 0$^*$ & 5.0 & 2.0 & 0.0 & 0.0 & 0.0 & 1.0 & 1.0 & 0.0 & -1.0 & -0.6 \\
 -12.5 & 0.5 & 0.5 & 0.0 & 0.0 & 7.5 & 2.0 & 3.0 & 0.0 & 0.0 & 1.0 & 1.0 & 0.5 & -1.0 & 0.0 \\
 5.0 & 1.0 & 0.0 & -0.2 & 0.2 & 1.0 & 1.0 & 0.5 & 0.4 & 0.0 & -5.0 & 1.0 & 2.0 & 0.0 & 0.0 \\
 7.5 & 1.75 & 0.0 & 0.0 & 0.0 & 1.0 & 1.0 & 1.5 & 0.4 & -0.4 & 1.0 & 1.0 & 0.5 & 0.4 & 0.2 \\\midrule
 \multicolumn{5}{c}{Cluster 10} & \multicolumn{5}{c}{Cluster 11} & \multicolumn{5}{c}{Cluster 12}   \\[1mm] \midrule
  $\kappa_{\lambda}$& $\kappa_{t}$ & $c_2$ & $c_g$ & $c_{2g}$ & $\kappa_{\lambda}$& $\kappa_{t}$ & $c_2$ & $c_g$ & $c_{2g}$& $\kappa_{\lambda}$& $\kappa_{t}$ & $c_2$ & $c_g$ & $c_{2g}$ \\
5.0& 1.0& 0.0 & -0.4& 0.4  & 5.0 & 2.0 & 1.0 & 0.0 & 0.0 & 3.5 & 0.75 & 0.5 & 0.0 & 0.0 \\
-7.5 & 0.5 & 0.5 & 0.0 & 0.0 & -2.4 & 2.5 & 3.0 & 0.0 & 0.0 & -5.0 & 1.0 & -1.0 & 0.0 & 0.0 \\
-12.5 & 1.5 & 3.0 & 0.0 & 0.0 & -3.5 & 2.0 & 2.0 & 0.0 & 0.0 & -2.4 & 2.5 & 1.0 & 0.0 & 0.0 \\
15.0 & 1.0 & -2.0 & 0.0 & 0.0 & -3.5 & 2.5 & 3.0 & 0.0 & 0.0 & 7.5 & 1.0 & 0.0 & 0.6 & -0.6 \\
-5.0 & 0.5 & 0.5 & 0.0 & 0.0 & -5 & 2.0 & 3.0 & 0.0 & 0.0 & 7.5 & 1.5 & 0.5 & 0.0 & 0.0 \\
-10.0 & 1.0 & 2.0 & 0.0 & 0.0 & -10.0 & 1.5 & 3.0 & 0.0 & 0.0 & -15.0 & 2.5 & 3.0 & 0.0 & 0.0 \\
\bottomrule
\end{tabular}
}
\caption{The parameter space coordinates of the outliers of the clusters whose
benchmarks are in Table~\ref{tab:bench}. 
\label{tab:out}}
\end{table}

\clearpage
\subsection{Experimental results from LHC Run I data taking period}

Recently both ATLAS and CMS collaborations performed searches for the 
non resonant production of Higgs boson pairs with 8\,TeV LHC data~\cite{Aad:2014yja, Aad:2015xja,  Aad:2015uka,  Khachatryan:2016sey}. 
The ATLAS collaboration considered only the SM-like kinematics for the signal.
The best upper limit of $\sigmaHH<0.69$\,pb is obtained in Ref.~\cite{Aad:2015xja} as a results of a combination of the four channels
$\HH \to \tau\tau\,b\bar{b}$, $\HH \to \gamma\gamma\,b\bar{b}$, $\HH \to b\bar{b}\,b\bar{b}$ and $\HH \to \gamma\gamma\,WW$. %observed 
%an upper limit of 0.69 pb on $\HH$ production rate.  
For the same hypothesis, the CMS collaboration provides a limit of $\sigmaHH<0.71$\,pb based on the results from the
$\HH \to \gamma\gamma\,b\bar{b}$ channel~\cite{Khachatryan:2016sey}. 

Reference~\cite{Khachatryan:2016sey} pushes further the exploration of the BSM parameter space for non-resonant $\HH$ production, by varying a subset of the parameter space, given by  $\kappa_{\lambda} ,\kappa_t $ and $c_2$. All in all, a grid of 124 points was generated. First a scan of $\kappa_{\lambda}$ was performed: $\kappa_{\lambda} = \pm$20, $\pm$15, $\pm$10, $\pm$5, 2.4, 1 (the SM point) and 0. In addition eight two-dimensional scans were done in the plane $(c_2,\kappa_t)$, for fixed values  of  $\kappa_{\lambda} = \pm$20, $\pm$15, $\pm$10, 1 and 0. In those, $c_2 = \pm$3, $\pm$2,  0 and  $\kappa_t = $ 0.75, 1, 1.25 were considered.  
One may notice that the scan in the $\kappa_t$ variable covers a smaller range than the scan that defined the clusters, but with a finer granularity.

The signals are searched for in two regions of $\mHH$, $<350$ and $\mHH >350$\,GeV, optimized to maximize the sensitivity for the SM-like search.
The observed limits on $\sigmaHH$ span between 1.36\,pb and 4.42\,pb depending on the point of the phase-space. By itself this result shows the 
importance of the kinematics of the BSM non-resonant production. 

The particularity of the $\HH \to \gamma\gamma\,b\bar{b}$ channel is to provide an excellent reconstruction of $\mHH$ with a resolution 
of $10-20$\,GeV and a rather constant signal efficiency for $250 < \mHH < 1000$\,GeV varying between 20\% and 30\%. 
Therefore this channel is well suited to resolve the details of the $\mHH$ spectrum and to challenge the cluster approach. This is what we discuss
in the following by applying the clustering technique to the analyzed parameter space.


From the 124 parameter space points for which we have experimental limits, only $N_{\rm samples } = 31$ coincide exactly with any of the parameter space points used to determine the clusters. However we note that other $N_{\rm samples} = 22$ extra points lie in between points that belong to the same cluster, while the gradient of cross section between them is smooth. This allows one to tag those intermediate points as belonging to the same cluster. 
As an example we show in Fig.~\ref{fig:temp_aabb} the distribution of the points used for the cluster definition in two-dimensional scans in 
 $(c_2,\kappa_t)$, for fixed values  of  $\kappa_{\lambda} = \pm$ 15 and $\pm$10. 
 Following the above defined algorithm the point $(\kappa_{\lambda} ,\kappa_t, c_2) = (15, 1.25, -2)$ is assigned as belonging to cluster 10. Similarly the point $(\kappa_{\lambda} ,\kappa_t, c_2) = (15, 0.75, -2)$  is not assigned to any cluster\footnote{Strictly speaking to assign those \textit{frontier} clusters we shall include them into the clustering procedure.}. 


\begin{figure}[hbt]\begin{center}
\includegraphics[width=1.0\textwidth, angle =0 ]{clusters5D_clu_noc2_12_1057_aabb.pdf}
\caption{\small Distribution of points in the $c_2 \times \kappa_t$ plane for different values of $\kappa_{\lambda}$ when $(c_g,\, c_{2g}) = (0,0)$.
Circles describe clusters whose benchmark has Higgs boson $p_T$ ($\pTH$) peaking around 100\,GeV. Downward-pointing triangles describe clusters where $\pTH$ is peaking around 50\,GeV or less, while upward-pointing triangles describe ones with $\pTH$ peaking around 150\,GeV or more. Finally, crosses describe clusters that show a double peaking structure in the $\pTH$ distribution. 
Larger markers indicate benchmark points. The gray lines correspond to iso-contours of constant cross section $\sigmaHH$.
See Fig.~8 in Ref.~\cite{Dall'Osso:2015aia} for more details. 
\label{fig:temp_aabb}}
\end{center}\end{figure}

\begin{figure}[hbt]\begin{center}
\includegraphics[width=1.1\textwidth, angle =0 ]{limits_points_1D.pdf}
\caption{\small Experimental limits from $\HH\to \gamma\gamma\,b\bar{b}$ search performed by the CMS collaboration~\cite{Khachatryan:2016sey}, organized by clusters following the procedure described in the text.  
The blue points correspond to the 95\% CL expected limits, while the green and yellow bands visualize one and two standard deviations around the latter.
\label{fig:lim_aabb}}
\end{center}\end{figure}

In Fig.~\ref{fig:lim_aabb} we show a total of 53 experimental limits at 95\% CL, organized by clusters. 
Unfortunately not all the clusters are equally populated and the statistics ranges between 0 and 19 samples. 
Still we have enough information to derive the first conclusions.

Table~\ref{tab:mean} contains the mean values of the expected and observed experimental limits for each cluster and the standard deviations, defined with respect to the mean value. The same information is displayed in Fig.~\ref{fig:mean_mass}, for the observed limits only. 
As expected the largest limits correspond to threshold-like clusters, for instance cluster 7 and cluster 10.   
Clusters 4 and 12 seem to exhibit two sub-clusters each.  In the figure we also include the values of the medians. This estimator is less affected by the outliers than the mean. We observe that mean and median are close to each other in most cases.

As the observed limits are more susceptible to small data fluctuations their variance is bigger than the spread of the expected limits.  
The standard deviation derived for each cluster should be taken with care, as the parameter space scan in Ref.~\cite{Khachatryan:2016sey} was not done in a systematic way regarding the signal kinematic properties. 
For most of the clusters the relative size of the standard deviation does not exceed 5-10\%. For cluster 1 and 10 it increases up to 20\%. In Fig.~\ref{fig:out_mass_exp} we show the comparison of the $\mHH$ distributions. We observed as expected that the largest difference in limits corresponds to the largest difference in shapes. Therefore reweighting the benchmark to the outliers is an important element of an experimental analysis using this cluster technique.

By eye we see that the intra-cluster variance ($V_{\rm Intra, i}$) is smaller than the variance of limits between clusters (inter-cluster variance $V_{\rm Inter, i}$). 
To provide a more quantitative estimate of this phenomenon we use the Fisher-Snedecor test quite commonly used in biology for example to assess the compatibility of two medical tests. It is implemented via 

\begin{equation}
{\rm p}\mbox{-}{\rm value} = {\rm TMath::FDist}(V_{\rm Inter}/V_{\rm Intra, i}, N_{clus}, \#{\rm samples}). 
\end{equation}

It uses the ratio of inter-cluster variance and intra-cluster variance for each cluster. The number of degrees of freedom of the numerator is assumed to be $N_{clus} = 8$ and the denominator is the number of samples. The output of this function is a p-value on the hypothesis that both variances are statistically compatible. The results are provided in Table~\ref{tab:mean}. We observe that the clustering procedure is successful to reduce the variance of the phase-space and identify groups with similar experimental behavior in the complex phase-space of $\HH$ production final state.


\begin{table}[h]
\centering
\small{
\begin{tabular}{rcccccccc| c}
\toprule
Benchmark & 1  & 3 & 4 & 5  & 7  & 9 & 10  & 12 & All \\[1.5mm]
\midrule
\# samples  & 3 (1) & 3 (2) & 13 (4) & 2 (1) & 8 (5) & 9 (6) & 5 (2) & 19 (10) & 8 Means \\[1.5mm]
\midrule
%$N_{\mbox{samples}}^{\mbox{ interpolated}}$ & 1 & 2 & 4 & 1 & 5 &  6 & 2 & 10 \\[1mm]\hline
%Obs. Median  (pb) & 1.98 & 1.75 & 1.95 & 1.34 & 4.12 & 1.37 & 3.53 & 2.86 & 1.97 \\[1.5mm]
Obs. Mean  (pb) & 1.92 & 1.75 & 1.87 & 1.34 & 4.08 & 1.39 & 3.63 & 2.69 & 2.33 \\[1.5mm]
$\sqrt{\mbox{Variance}}$ (pb) & 0.55 & 0.11 & 0.22 & 0.03 & 0.19 & 0.05 & 0.53 & 0.41 & 1.03 \\[1.5mm]
FS p-value & 6e-02 & 3e-05 & 6e-07 & 7e-07 & 5e-06 & 1e-12 & 4e-02 & 5e-04 & \\[1.5mm]
\midrule

%Exp. Median (pb) & 1.48 & 1.56 & 1.55 & 1.15 & 2.85 & 1.17 & 2.46 & 2.09 & 1.56 \\[1.5mm]
Exp. Mean (pb) & 1.51 & 1.52 & 1.61 & 1.1484 & 2.84 & 1.18 & 2.39 & 2.18 & 1.80\\[1.5mm]
$\sqrt{\mbox{Variance}}$ (pb) & 0.30 & 0.08 & 0.15 & 0.005 & 0.09 & 0.04 & 0.32 & 0.25 & 0.61 \\[1.5mm]
FS p-value & 4e-02 & 8e-05 & 3e-06 & 4e-09 & 5e-07 & 3e-11 & 4e-02 & 6e-04 & \\[1.5mm]
\bottomrule
\end{tabular} 
}
\caption{\small Mean and standard deviations of the expected and observed limits for the 8 clusters analyzed in the $\HH\to \gamma\gamma\,b\bar{b}$ search performed by CMS collaboration. The label "\# samples" denotes the number of samples identified per cluster. The number in parentheses indicates how many of these were identified to be in the cluster from interpolation, as described in the text.  
The last column shows the total unweighted mean and the associated standard deviation between the means of the 8 clusters. The Fisher-Snedecor p-values are also provided.
\label{tab:mean}}
\end{table}


\begin{figure}[hbt]\begin{center}
\includegraphics[width=0.4\textwidth, angle =0 ]{aabb/Mean_variance.pdf}
\caption{\small Experimental limits from the $\HH \to \gamma\gamma\,b\bar{b}$ analysis performed by the CMS collaboration~\cite{Khachatryan:2016sey}, organized by clusters; see text for details.   \label{fig:mean_mass}}
\end{center}\end{figure}



\begin{figure}[hbt]\begin{center}
\includegraphics[width=0.42\textwidth, angle =0 ]{aabb/5par_13Tev_Nclu12_Clus1_mhh.pdf}
\includegraphics[width=0.42\textwidth, angle =0 ]{aabb/5par_13Tev_Nclu12_Clus10_mhh.pdf}
\caption{\small The $\mHH$ distribution of the samples in cluster 1 and 10. The benchmark (black line) is compared with the 
points studied by~\cite{Khachatryan:2016sey} (bold color red and blue lines) that coincide with those considered in~\cite{Dall'Osso:2015aia}. \label{fig:out_mass_exp}}
\end{center}\end{figure}


